Vera: A General-Purpose Plausibility Estimation Model for Commonsense Statements

Despite the much discussed capabilities of today's language models, they are still prone to silly and unexpected commonsense failures. We consider a retrospective verification approach that reflects on the correctness of LM outputs, and introduce Vera, a general-purpose model that estimates the plausibility of declarative statements based on commonsense knowledge. Trained on ~7M commonsense statements created from 19 QA datasets and two large-scale knowledge bases, and with a combination of three training objectives, Vera is a versatile model that effectively separates correct from incorrect statements across diverse commonsense domains. When applied to solving commonsense problems in the verification format, Vera substantially outperforms existing models that can be repurposed for commonsense verification, and it further exhibits generalization capabilities to unseen tasks and provides well-calibrated outputs. We find that Vera excels at filtering LM-generated commonsense knowledge and is useful in detecting erroneous commonsense statements generated by models like ChatGPT in real-world settings.

==> floats/results_acc.tex <==
\begin{figure*}[t]
\centering
% This image is generated by `python visualize_acc.py`
\includegraphics[width=0.95\linewidth]{images/results_acc.png}
\caption{
    Results on commonsense problem-solving in the verification format, with \methodname{} and baseline models.
    See \autoref{fig:results_probsolving} for detailed results and explanations.
}
\label{fig:results_acc}
% \vspace{-16pt}
\end{figure*}

==> floats/results_chatgpt_failures_metrics.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{3pt}
\centering
\resizebox{0.5 \textwidth}{!}{%
\begin{tabular}{l c}
\toprule
\textbf{Metric} & \textbf{Value} \\
\midrule
Precision (incorrect statements) & 0.91 \\
Recall (incorrect statements) & 0.74 \\
$F_1$ (incorrect statements) & 0.82 \\
Classification accuracy on incorrect statements & 0.74 \\
Classification accuracy on correct statements & 0.93 \\
Classification accuracy on paired statements & 0.74 \\
\bottomrule
\end{tabular}
}%
\caption{
    Results on using \methodname{} to detect commonsense mistakes made by ChatGPT.
}
\label{tab:results_chatgpt_failures_metrics}
% \vspace{-8pt}
\end{table*}


==> floats/trash/results_bool.tex <==
\begin{table*}[!h]
\setlength{\tabcolsep}{2pt}
\centering
\resizebox{0.4 \textwidth}{!}{%
% \begin{tabular}{l cccc}
% \toprule
% \textbf{Dataset} $\rightarrow$ & \multicolumn{2}{c}{\textbf{Avg}} & \multicolumn{2}{c}{CSQA2} \\
% & Acc & ECE & Acc & ECE \\
% \midrule
% I2D2 Critic (125M) & {gengen-iter-2} \\
% UnifiedQA-v2 (11B) & {allenai/unifiedqa-v2-t5-11b-1251000} \\
% Entailer (11B) & {allenai/entailer-11b} \\
% GPT-3.5 (175B) & {openai/text-davinci-002} \\
% Flan-T5 (11B) & {google/flan-t5-xxl} \\
% \midrule
% \methodname{}-LLaMA (7B) & {ours-llama} \\
% \methodname{}-T5v1.1-XXL (6B) & {ours-t5} \\
% \methodname{}-FlanT5-XXL (6B) & {ours-flan-t5} \\
% \bottomrule
% \end{tabular}
\begin{tabular}{l cccc}
\toprule
\textbf{Dataset} $\rightarrow$ & \multicolumn{2}{c}{\textbf{Avg}} & \multicolumn{2}{c}{CSQA2} \\
& Acc & ECE & Acc & ECE \\
\midrule
I2D2 Critic (125M) & 43.65 & 16.68 & 43.65 & 16.68 \\
UnifiedQA-v2 (11B) & 56.05 & 8.23 & 56.05 & 8.23 \\
Entailer (11B) & 56.00 & 13.03 & 56.00 & 13.03 \\
GPT-3.5 (175B) & 58.00 & 14.90 & 58.00 & 14.90 \\
Flan-T5 (11B) & 62.25 & 9.54 & 62.25 & 9.54 \\
\midrule
\methodname{}-LLaMA (7B) & 62.60 & 9.81 & 62.60 & 9.81 \\
\methodname{}-T5v1.1-XXL (6B) & 68.60 & 6.75 & 68.60 & 6.75 \\
\methodname{}-FlanT5-XXL (6B) & 69.45 & 6.81 & 69.45 & 6.81 \\
\bottomrule
\end{tabular}
}%
% \vspace{-4pt}
\caption{
    Results on \textbf{seen} \textbf{boolean} datasets.
    Accuracy on the dev set is reported.
    Model predictions are calibrated before ECE is computed.
}
\label{tab:results_bool_seen}
\vspace{12pt}
\resizebox{0.4 \textwidth}{!}{%
% \begin{tabular}{l cccc}
% \toprule
% \textbf{Dataset} $\rightarrow$ & \multicolumn{2}{c}{\textbf{Avg}} & \multicolumn{2}{c}{SpatialCS} \\
% & Acc & ECE & Acc & ECE \\
% \midrule
% I2D2 Critic (125M) & {gengen-iter-2} \\
% UnifiedQA-v2 (11B) & {allenai/unifiedqa-v2-t5-11b-1251000} \\
% Entailer (11B) & {allenai/entailer-11b} \\
% GPT-3.5 (175B) & {openai/text-davinci-002} \\
% Flan-T5 (11B) & {google/flan-t5-xxl} \\
% \midrule
% \methodname{}-LLaMA (7B) & {ours-llama} \\
% \methodname{}-T5v1.1-XXL (6B) & {ours-t5} \\
% \methodname{}-FlanT5-XXL (6B) & {ours-flan-t5} \\
% \bottomrule
% \end{tabular}
\begin{tabular}{l cccc}
\toprule
\textbf{Dataset} $\rightarrow$ & \multicolumn{2}{c}{\textbf{Avg}} & \multicolumn{2}{c}{SpatialCS} \\
& Acc & ECE & Acc & ECE \\
\midrule
I2D2 Critic (125M) & 56.22 & 12.05 & 56.22 & 12.05 \\
UnifiedQA-v2 (11B) & 78.25 & 12.40 & 78.25 & 12.40 \\
Entailer (11B) & 85.15 & 15.80 & 85.15 & 15.80 \\
GPT-3.5 (175B) & 77.49 & 3.32 & 77.49 & 3.32 \\
Flan-T5 (11B) & 95.23 & 11.01 & 95.23 & 11.01 \\
\midrule
\methodname{}-LLaMA (7B) & 85.29 & 5.07 & 85.29 & 5.07 \\
\methodname{}-T5v1.1-XXL (6B) & 93.44 & 6.45 & 93.44 & 6.45 \\
\methodname{}-FlanT5-XXL (6B) & 91.02 & 6.37 & 91.02 & 6.37 \\
\bottomrule
\end{tabular}
}%
% \vspace{-4pt}
\caption{
    Results on \textbf{unseen} \textbf{boolean} datasets.
    Accuracy on the dev set is reported.
    Model predictions are calibrated before ECE is computed.
}
\label{tab:results_bool_unseen}
\end{table*}

==> floats/trash/results_mc.tex <==
\begin{table*}[!h]
\setlength{\tabcolsep}{2pt}
\centering
\resizebox{\textwidth}{!}{%
% \begin{tabular}{l cccccccccc ccccccc}
% \toprule
% \textbf{Dataset} $\rightarrow$ & \textbf{Avg} & OBQA & ARC\_e & ARC\_h & AI2Sci\_e & AI2Sci\_m & CSQA & QASC & PIQA & SIQA & WG & C2S & SciQ & QuaRel & QuaRTz & CycIC & ComVE \\
% \midrule
% I2D2 Critic (125M) & {gengen-iter-2} \\
% UnifiedQA-v2 (11B) & {allenai/unifiedqa-v2-t5-11b-1251000} \\
% Entailer (11B) & {allenai/entailer-11b} \\
% GPT-3.5 (175B) & {openai/text-davinci-002} \\
% Flan-T5 (11B) & {google/flan-t5-xxl} \\
% \midrule
% \methodname{}-LLaMA (7B) & {ours-llama} \\
% \methodname{}-T5v1.1-XXL (6B) & {ours-t5} \\
% \methodname{}-FlanT5-XXL (6B) & {ours-flan-t5} \\
% \bottomrule
% \end{tabular}
\begin{tabular}{l cccccccccc ccccccc}
\toprule
\textbf{Dataset} $\rightarrow$ & \textbf{Avg} & OBQA & ARC\_e & ARC\_h & AI2Sci\_e & AI2Sci\_m & CSQA & QASC & PIQA & SIQA & WG & C2S & SciQ & QuaRel & QuaRTz & CycIC & ComVE \\
\midrule
I2D2 Critic (125M) & 55.75 & 44.80 & 55.61 & 35.79 & 55.28 & 50.40 & 61.51 & 45.25 & 67.36 & 56.45 & 55.56 & 63.17 & 55.10 & 61.51 & 60.16 & 35.72 & 88.26 \\
UnifiedQA-v2 (11B) & 56.34 & 54.60 & 48.77 & 39.46 & 48.78 & 43.20 & 44.23 & 32.61 & 63.98 & 52.10 & 70.64 & 75.96 & 42.20 & 81.65 & 71.35 & 48.29 & 83.65 \\
Entailer (11B) & 74.90 & 74.40 & 81.93 & 64.88 & 77.24 & 82.40 & 67.81 & 57.56 & 78.78 & 64.33 & 77.11 & 82.86 & 76.90 & 85.97 & 76.56 & 52.81 & 96.89 \\
GPT-3.5 (175B) & 75.93 & 72.40 & 86.32 & 70.23 & 85.37 & 81.60 & 69.21 & 65.01 & 82.97 & 67.35 & 68.67 & 81.07 & 86.30 & 77.70 & 72.66 & 50.39 & 97.69 \\
Flan-T5 (11B) & 80.58 & 79.60 & 85.79 & 71.24 & 86.99 & 81.60 & 69.21 & 64.58 & 83.95 & 73.23 & 84.69 & 84.40 & 80.80 & 92.81 & 82.03 & 69.90 & 98.40 \\
\midrule
\methodname{}-LLaMA (7B) & 82.46 & 78.00 & 81.75 & 71.57 & 83.74 & 77.60 & 74.86 & 68.68 & 84.44 & 76.46 & 86.66 & 85.42 & 88.10 & 94.24 & 80.73 & 88.97 & 98.19 \\
\methodname{}-T5v1.1-XXL (6B) & 86.57 & 83.20 & 88.07 & 78.60 & 93.50 & 86.40 & 77.97 & 73.33 & 88.47 & 80.14 & 92.42 & 85.93 & 88.80 & 93.88 & 84.90 & 91.73 & 97.79 \\
\methodname{}-FlanT5-XXL (6B) & 86.30 & 82.60 & 87.02 & 77.59 & 92.68 & 88.00 & 77.89 & 70.95 & 88.47 & 80.14 & 91.95 & 87.72 & 87.60 & 94.96 & 85.16 & 89.53 & 98.50 \\
\bottomrule
\end{tabular}
}%
% \vspace{-4pt}
\caption{
    Results on \textbf{seen} \textbf{multiple-choice} datasets.
    Accuracy on the dev set is reported.
}
\label{tab:results_mc_seen}
\vspace{12pt}
\resizebox{0.5 \textwidth}{!}{%
% \begin{tabular}{l ccccc}
% \toprule
% \textbf{Dataset} $\rightarrow$ & \textbf{Avg} & WSC & COPA & NumerSense & PROST \\
% \midrule
% I2D2 Critic (125M) & {gengen-iter-2} \\
% UnifiedQA-v2 (11B) & {allenai/unifiedqa-v2-t5-11b-1251000} \\
% Entailer (11B) & {allenai/entailer-11b} \\
% GPT-3.5 (175B) & {openai/text-davinci-002} \\
% Flan-T5 (11B) & {google/flan-t5-xxl} \\
% \midrule
% \methodname{}-LLaMA (7B) & {ours-llama} \\
% \methodname{}-T5v1.1-XXL (6B) & {ours-t5} \\
% \methodname{}-FlanT5-XXL (6B) & {ours-flan-t5} \\
% \bottomrule
% \end{tabular}
\begin{tabular}{l ccccc}
\toprule
\textbf{Dataset} $\rightarrow$ & \textbf{Avg} & WSC & COPA & NumerSense & PROST \\
\midrule
I2D2 Critic (125M) & 54.43 & 80.59 & 72.80 & 35.00 & 29.35 \\
UnifiedQA-v2 (11B) & 55.10 & 71.79 & 81.20 & 35.00 & 32.40 \\
Entailer (11B) & 68.05 & 86.08 & 92.40 & 51.00 & 42.70 \\
GPT-3.5 (175B) & 70.04 & 83.15 & 88.80 & 67.50 & 40.70 \\
Flan-T5 (11B) & 73.22 & 90.48 & 93.00 & 57.50 & 51.90 \\
\midrule
\methodname{}-LLaMA (7B) & 71.19 & 90.48 & 87.80 & 58.00 & 48.50 \\
\methodname{}-T5v1.1-XXL (6B) & 78.70 & 94.51 & 93.40 & 66.50 & 60.40 \\
\methodname{}-FlanT5-XXL (6B) & 78.48 & 94.14 & 95.00 & 61.50 & 63.30 \\
\bottomrule
\end{tabular}
}%
% \vspace{-4pt}
\caption{
    Results on \textbf{unseen} \textbf{multiple-choice} datasets.
    Accuracy on the dev set is reported.
}
\label{tab:results_mc_unseen}
\end{table*}

==> floats/trash/results_ood.tex <==
\begin{table*}[!h]
\setlength{\tabcolsep}{2pt}
\centering
\resizebox{0.5 \textwidth}{!}{%
% \begin{tabular}{l cccccc}
% \toprule
% \textbf{Dataset} $\rightarrow$ & \textbf{Avg} & SWAG & HellaSwag & CODAH & SCT & $\alpha$NLI \\
% \midrule
% I2D2 Critic (125M) & {gengen-iter-2} \\
% UnifiedQA-v2 (11B) & {allenai/unifiedqa-v2-t5-11b-1251000} \\
% Entailer (11B) & {allenai/entailer-11b} \\
% GPT-3.5 (175B) & {openai/text-davinci-002} \\
% Flan-T5 (11B) & {google/flan-t5-xxl} \\
% \midrule
% \methodname{}-LLaMA (7B) & {ours-llama} \\
% \methodname{}-T5v1.1-XXL (6B) & {ours-t5} \\
% \methodname{}-FlanT5-XXL (6B) & {ours-flan-t5} \\
% \bottomrule
% \end{tabular}
\begin{tabular}{l cccccc}
\toprule
\textbf{Dataset} $\rightarrow$ & \textbf{Avg} & SWAG & HellaSwag & CODAH & SCT & $\alpha$NLI \\
\midrule
I2D2 Critic (125M) & 70.42 & 72.15 & 53.30 & 67.30 & 88.24 & 71.08 \\
UnifiedQA-v2 (11B) & 52.83 & 31.75 & 36.60 & 49.00 & 82.04 & 64.75 \\
Entailer (11B) & 70.63 & 52.45 & 47.65 & 80.70 & 94.39 & 77.94 \\
GPT-3.5 (175B) & 80.09 & 67.40 & 73.90 & 86.40 & 96.37 & 76.37 \\
Flan-T5 (11B) & 80.52 & 69.20 & 64.55 & 89.60 & 98.45 & 80.81 \\
\midrule
\methodname{}-LLaMA (7B) & 82.54 & 75.55 & 76.25 & 86.80 & 98.18 & 75.91 \\
\methodname{}-T5v1.1-XXL (6B) & 86.66 & 76.30 & 85.90 & 88.60 & 98.56 & 83.94 \\
\methodname{}-FlanT5-XXL (6B) & 86.59 & 77.35 & 84.60 & 88.70 & 98.82 & 83.49 \\
\bottomrule
\end{tabular}
}%
% \vspace{-4pt}
\caption{
    Results on \textbf{out-of-domain} \textbf{multiple-choice} datasets.
    Accuracy on the dev set is reported.
}
\label{tab:results_mc_ood}
\vspace{12pt}
\resizebox{0.5 \textwidth}{!}{%
% \begin{tabular}{l cccccc}
% \toprule
% \textbf{Dataset} $\rightarrow$ & \multicolumn{2}{c}{\textbf{Avg}} & \multicolumn{2}{c}{StrategyQA} & \multicolumn{2}{c}{CREAK} \\
% & Acc & ECE & Acc & ECE & Acc & ECE \\
% \midrule
% I2D2 Critic (125M) & {gengen-iter-2} \\
% UnifiedQA-v2 (11B) & {allenai/unifiedqa-v2-t5-11b-1251000} \\
% Entailer (11B) & {allenai/entailer-11b} \\
% GPT-3.5 (175B) & {openai/text-davinci-002} \\
% Flan-T5 (11B) & {google/flan-t5-xxl} \\
% \midrule
% \methodname{}-LLaMA (7B) & {ours-llama} \\
% \methodname{}-T5v1.1-XXL (6B) & {ours-t5} \\
% \methodname{}-FlanT5-XXL (6B) & {ours-flan-t5} \\
% \bottomrule
% \end{tabular}
\begin{tabular}{l cccccc}
\toprule
\textbf{Dataset} $\rightarrow$ & \multicolumn{2}{c}{\textbf{Avg}} & \multicolumn{2}{c}{StrategyQA} & \multicolumn{2}{c}{CREAK} \\
& Acc & ECE & Acc & ECE & Acc & ECE \\
\midrule
I2D2 Critic (125M) & 58.84 & 7.35 & 52.40 & 8.61 & 65.28 & 6.08 \\
UnifiedQA-v2 (11B) & 56.77 & 8.34 & 49.34 & 13.11 & 64.19 & 3.56 \\
Entailer (11B) & 70.94 & 11.52 & 60.26 & 16.95 & 81.62 & 6.09 \\
GPT-3.5 (175B) & 71.53 & 13.07 & 56.77 & 21.64 & 86.29 & 4.50 \\
Flan-T5 (11B) & 74.81 & 11.15 & 61.14 & 14.91 & 88.48 & 7.39 \\
\midrule
\methodname{}-LLaMA (7B) & 74.18 & 8.99 & 64.19 & 11.45 & 84.17 & 6.53 \\
\methodname{}-T5v1.1-XXL (6B) & 75.13 & 7.80 & 65.07 & 10.43 & 85.19 & 5.18 \\
\methodname{}-FlanT5-XXL (6B) & 73.78 & 8.00 & 64.19 & 12.03 & 83.37 & 3.97 \\
\bottomrule
\end{tabular}
}%
% \vspace{-4pt}
\caption{
    Results on \textbf{out-of-domain} \textbf{boolean} datasets.
    Accuracy on the dev set is reported.
}
\label{tab:results_bool_ood}
\end{table*}

==> sections/ethics.tex <==
\section*{Ethics Statement}
\label{sec:ethics}
